APEX: An Extensible Model for Agent-Assisted Production Scheduling

Production scheduling requires realistic models that reflect operational constraints and efficient methods that balance competing goals. Putting these methods into use also requires data integration, model adaptation and specialist expertise. We present APEX, an extensible production scheduling framework built around a general model and hybrid multiobjective search. Agent assistance supports both scheduling and model refinement: agents prepare data and explore scenarios in natural language, while coding agents help implement and test new constraints and objectives. Shared construction and checking procedures connect these adaptations to the scheduling core. We benchmark eight APEX configurations against NSGA-II, SPEA2, MOEA/D and SMS-EMOA on 69 public job-shop, flexible job-shop and permutation flow-shop instances, assessing workload completion time (makespan), total job flowtime and computation time. Hybrid configurations achieve the best aggregate solution quality, although the leading method depends on the problem class and objective. A separate synthetic workflow study uses OpenAI's GPT-6-astra as an interaction layer between the human planner and the algorithmic core, testing rule additions, plan and objective changes, and what-if comparisons. All 24 sessions completed the requested changes and passed independent checks of saved models and schedules. A separate coding evaluation produced six native implementations of an additional objective or hard constraint through predefined extension hooks. All passed independent checks without modifying the core.

==> tables/native-extension.tex <==
\begin{tabularx}{\textwidth}{@{}Xrrr@{}}
\toprule
New implementation & Complete & Checks per pass & Median time (s) \\
\midrule
Squared-tardiness objective & 3/3 & 68 & 198.0 \\
Exposure-balance constraint & 2/3 & 61 & 249.6 \\
\bottomrule
\end{tabularx}


==> tables/workflow-development.tex <==
\begin{tabular}{@{}lrr@{}}
\toprule
Measure & Earlier matched tasks & Follow-up \\
\midrule
Completed workflows & 23/24 & 24/24 \\
Correct saved candidates & 24/24 & 24/24 \\
Timeouts & 1 & 0 \\
Native argument errors & 26 & 0 \\
Median session time (s) & 78.5 & 44.5 \\
Median tool calls & 15 & 7 \\
Median internal XH time (ms) & 15.8 & 16.7 \\
Sessions with token records & 23/24 & 24/24 \\
Median input tokens & 314,664.0 & 163,176.5 \\
Median output tokens & 1,606.0 & 770.5 \\
\bottomrule
\end{tabular}


==> tables/workflow-followup.tex <==
\begin{tabularx}{\textwidth}{@{}lXrrr@{}}
\toprule
Workflow & Requested change & Passes & MS (s) & Cost \\
\midrule
Rules & M1 unavailable on $[0,2400)$ & 3/3 & 6,300 & 30 \\
 & J3-2 within $[7200,10800]$ & 3/3 & 9,300 & 30 \\
Plans & J2-1 on M2 at $3600$ & 3/3 & 8,400 & 30 \\
 & Freeze baseline starts before $1800$ & 3/3 & 4,800 & 30 \\
Objectives & Tardiness first, then makespan & 3/3 & 4,800 & 30 \\
 & Mode cost first, then makespan & 3/3 & 9,000 & 12 \\
What-if & M3 outage on $[0,3600)$; compare & 3/3 & 5,700 & 27 \\
 & Earlier due date and higher priority; compare & 3/3 & 4,800 & 30 \\
\bottomrule
\end{tabularx}


==> tables/xe.tex <==
\begin{tabular}{llrrrr}
\toprule
Class & Variant & HV (\%) & MS (\%) & FT (\%) & Time (s) \\
\midrule
JSP & NSGA-II (historical) & \textbf{1.207} & \textbf{1.38} & \textbf{6.18} & \textbf{0.167} \\
JSP & XE original & 4.997 & 16.19 & 8.73 & 0.714 \\
JSP & XE refined, 16 & 3.622 & 11.88 & 6.33 & 0.794 \\
JSP & XE refined, 64 & 4.445 & 13.62 & 9.68 & 0.809 \\
FJSP & NSGA-II (historical) & 4.774 & \textbf{17.60} & 29.06 & \textbf{0.269} \\
FJSP & XE original & 4.847 & 23.69 & 19.30 & 0.974 \\
FJSP & XE refined, 16 & \textbf{3.912} & 19.69 & \textbf{15.10} & 1.135 \\
FJSP & XE refined, 64 & 5.204 & 25.87 & 20.17 & 1.101 \\
PFSP & NSGA-II (historical) & 1.273 & 3.16 & 4.00 & \textbf{0.131} \\
PFSP & XE original & 0.928 & 2.40 & 3.16 & 8.745 \\
PFSP & XE refined, 16 & \textbf{0.321} & \textbf{1.24} & \textbf{1.26} & 8.715 \\
PFSP & XE refined, 64 & 0.760 & 1.97 & 2.80 & 9.115 \\
\bottomrule
\end{tabular}

